Test-Time Preference Optimization: On-the-Fly Alignment via Iterative Textual Feedback

Large language models (LLMs) demonstrate impressive performance but lack the flexibility to adapt to human preferences quickly without retraining. In this work, we introduce Test-time Preference Optimization (TPO), a framework that aligns LLM outputs with human preferences during inference, removing the need to update model parameters. Rather than relying on purely numerical rewards, TPO translates reward signals into textual critiques and uses them as textual rewards to iteratively refine its response. Evaluations on benchmarks covering instruction following, preference alignment, safety, and mathematics reveal that TPO progressively improves alignment with human preferences. Notably, after only a few TPO steps, the initially unaligned Llama-3.1-70B-SFT model can surpass the aligned counterpart, Llama-3.1-70B-Instruct. Furthermore, TPO scales efficiently with both the search width and depth during inference. Through case studies, we illustrate how TPO exploits the innate capacity of LLM to interpret and act upon reward signals. Our findings establish TPO as a practical, lightweight alternative for test-time preference optimization, achieving alignment on the fly. Our code is publicly available at https://github.com/yafuly/TPO.

==> sections/method_bkp.tex <==

\paragraph{Variable Definition.}
In TextGrad, the \emph{response variable} $v$ represents the response associated with a query $x$. 
Unlike traditional gradient descent methods, which optimize continuous parameters $\theta$ (e.g., neural weights of size $512 \times 512$), TextGrad treats the response itself as the variable to be refined. 
Instead of fine-tuning the model parameters $\theta$ to produce an optimal response, the optimization focuses directly on improving $v$. 
Initially, $v$ can be obtained through a call to a large language model (LLM), for instance:
\[
v 
\;=\;
% \;\leftarrow\; 
\text{LLM}(x).
\]



\paragraph{Loss Function.}
Traditional gradient descent methods define continuous loss functions, e.g., cross-entropy loss, to measure the quality of generations. 
In contrast, TextGrad defines a test-time loss $\mathcal{L}(x, v)$ that quantifies how well the response $v$ addresses the query $x$. 
Unlike standard loss functions, $\mathcal{L}$ need not rely on ground-truth labels. 
Instead, it can incorporate textual instructions, style guidelines, or preference heuristics to prompt an LLM for critiques. 
For example:
\[
\mathcal{L}(x, v) \;=\; \text{LLM}\Bigl(
    % \begin{array}{l}
        \text{\small ``Critique how $v$ addresses $x$.''} \\
        % \text{\small Provide numeric or textual feedback.''}
    % \end{array}
\Bigr).
\]
This flexible formulation allows TextGrad to optimize outputs based on diverse qualitative criteria, such as correctness, clarity, or adherence to specific constraints, enabling fine-grained control over generated responses.


\paragraph{Gradient Computation.}
In conventional gradient descent, $\nabla_v \mathcal{L}(x, v)$ is a numerical vector. 
TextGrad replaces this with \emph{textual} feedback:
\begin{equation}
\label{eq:textgrad_gradient}
\frac{\partial \mathcal{L}}{\partial v} 
% \;\equiv\;
\;=\;
\text{LLM}\Bigl(
\text{\small ``How to improve $v$ given $\mathcal{L}(x, v)$.''} \Bigr),
\end{equation}
where a call of LLM produces human-readable suggestions or criticisms for improving $v$. 
Although it is denoted as $\frac{\partial \mathcal{L}}{\partial v}$ for analogy, it is not a true \emph{numeric} gradient but rather an interpretive textual signal.

\paragraph{Variable Optimization.}
A standard numerical update (Equation~\ref{eq:vanilla_gd}) uses
\(\theta \leftarrow \theta - \alpha \,\nabla_\theta \mathcal{L}\).
By comparison, TextGrad's update step:
\begin{equation}
\label{eq:textgrad_update}
v_{\mathrm{new}}
\;=\;
\text{LLM}\Bigl(
\text{\small ``Improve $v$ given $\frac{\partial \mathcal{L}}{\partial v}$.''} 
\Bigr)
% \mathrm{TGD.step}\Bigl(v,\; \tfrac{\partial \mathcal{L}}{\partial v}\Bigr)
\end{equation}
replaces numeric subtraction with an LLM-based editing process. 

In summary, a complete iteration of TextGrad involves three LLM calls to emulate the steps of gradient descent: generating a critique, deriving a textual gradient, and applying the gradient to update the variable.

\subsubsection{Test-time Training} 



\paragraph{Interpretability \& Flexibility.}
TextGrad's reliance on textual feedback confers two main benefits:
\begin{itemize}
\item \emph{Interpretability:} Developers or end-users can read each “gradient” as a natural language critique, providing explicit insights into how and why the solution is revised.
\item \emph{Flexibility:} The “loss” can incorporate broad, potentially subjective criteria (e.g., clarity, correctness, style) that are challenging to encode as purely numeric differentiable functions.
\end{itemize}

\paragraph{Connection to Preference Optimization.}
Where RLHF and DPO (\S\ref{sec:preference_optimization}) focus on adjusting the model parameters $\theta$ to favor certain outputs, \emph{TextGrad} fine-tunes the \emph{output} itself at inference time. Hence, it complements or replaces conventional training-phase alignment by enabling on-the-fly revisions of solutions, without requiring additional model fine-tuning.

\medskip
\noindent
This methodology underpins our proposed \textit{Test-Time Preference Optimization} (\S\ref{sec:our_method}), where we apply TextGrad to dynamically refine responses based on user-specific or scenario-specific criteria.





==> tables/winrate.tex <==
     
\begin{table*}[t]
\caption{Win-rate against BoN.}
\label{tab:mtbench}
\vskip 0.15in
\begin{center}
\begin{small}
\begin{sc}                
        \setlength{\tabcolsep}{3pt} 
        \begin{tabular}{ccccc}  
            \toprule  
            \textbf{Model} & \textbf{AlpacaEval 2} & \textbf{ArenaHard} & \textbf{HH-RLHF}  & \textbf{Average} \\
            % Claude & & & \\
            % \midrule
            % \multicolumn{6}{c}{Win-rate against BoN30} \\
            % \midrule
            % \midrule
            % \multicolumn{6}{c}{Win-rate against BoN30} \\
            \midrule
            Llama-3.1-70B-SFT-TPO & & & &  \\
            % Llama-3.1-70B-SFT-TPO-Static & & & & & \\
            % \noalign{\vskip 1.5pt}\hdashline\noalign{\vskip 1.5pt}
            Llama-3.1-70B-Instrcut-TPO & & & &  \\
            % Llama-3.1-70B-Instrcut-TPO-Static & & & & &  \\
            Mistral-Small-TPO & & & &   \\
            \bottomrule
\end{tabular}
\end{sc}
\end{small}
\end{center}
\vskip -0.1in
\end{table*}
